An Enhanced Decoding Algorithm for Coded Compressed Sensing with Applications to Unsourced Random Access

Unsourced random access (URA) has emerged as a pragmatic framework for next-generation distributed sensor networks. Within URA, concatenated coding structures are often employed to ensure that the central base station can accurately recover the set of sent codewords during a given transmission period. Many URA algorithms employ independent inner and outer decoders, which can help reduce computational complexity at the expense of a decay in performance. In this article, an enhanced decoding algorithm is presented for a concatenated coding structure consisting of a wide range of inner codes and an outer tree-based code. It is shown that this algorithmic enhancement has the potential to simultaneously improve error performance and decrease the computational complexity of the decoder. This enhanced decoding algorithm is applied to two existing URA algorithms and the performance benefits of the algorithm are characterized. Findings are supported by numerical simulations.

==> IEEEabrv.tex <==
@comment{This file has been generated by Pybliographer}
@String{ tmc    = "IEEE Trans. Mobile Comput."}
@String{ ieeetcad   = "IEEE Transactions on Computer Aided Design"}
@String{ ptl    = {IEEE Photon.~Technol.~Lett.}}
@String{ tip    = {IEEE Trans.~Image Processing}}
@String{ commag     = {IEEE Commun. Mag.}}
@String{ mna    = "Mobile Networks and Applications"}
@String{ jssc   = "IEEE Journal of Solid-State Circuits"}
@String{ ieee   = "IEEE Press"}
@String{ transvlsi  = "IEEE Trans.~VLSI"}
@String{ vtc    = {Proc.~Vehicular Tech.~Conf.}}
@String{ cup    = "Cambridge University Press"}
@String{ acmtms     = {ACM Trans.~Math.~Software}}
@String{ issse  = "Proc. Intern. Symposium. on Signals, Systems and Elec."}
@String{ tsp    = {IEEE Trans.~Signal Processing}}
@String{ ta     = "(To appear)"}
@String{ mor    = "Mathematics of Operations Research"}
@String{ piee   = {IEE~Proc. Commun.}}
@String{ ieice  = "IEICE Trans. Fundam. of Elect., Commun. and Comp. Sciences"}
@String{ bstj   = {Bell System Tech.~J.}}
@String{ accepted   = "(Accepted)"}
@String{ aes    = {IEEE Transactions on Aerospace and Electronic Systems}}
@String{ sigcomm    = "Proc.~ACM Conference of the Special Interest Group on Data Communication (SIGCOMM)"}
@String{ tpami  = {IEEE Trans.~Patt.~Anal.~Machine Intell.}}
@String{ mit    = "MIT Press"}
@String{ el     = {IEE Electronics Letters}}
@String{ transcomp  = "IEEE Trans.~Computers"}
@String{ isssta     = "Proc.~IEEE Intn'l. Conf.~Spread Spectrum Tech. and Applications"}
@String{ icsp   = "IEEE Computer Society Press"}
@String{ tvt    = {IEEE Trans.~Veh.~Tech.}}
@String{ mobihoc    = "Proc.~ACM~Int.~Symp.~on~Mobile~Ad~Hoc~Network.~and~Comput. (MOBIHOC)"}
@String{ comml  = {IEEE Commun. Letters}}
@String{ josab  = {J.~Opt.~Soc.~Amer.~B}}
@String{ esp    = "Elsevier Science Publishers"}
@String{ icc    = "Proc.~IEEE International Conf.~Commun."}
@String{ cwi    = "CWI"}
@String{ tassp  = {IEEE Trans.~Acoust., Speech, Singal Processing}}
@String{ mgh    = "McGraw-Hill"}
@String{ annals = {Annals of Telecommun.}}
@String{ jsac   = {IEEE J.~Select.~Areas Commun.}}
@String{ icassp  = "Proc.~Intl. Conf. Acoustics Speech and Sig. Proc."}
@String{ jstqe  = {IEEE J. Select. Topics Quantum Electron.}}
@String{ jtcom  = {IEICE Trans.~Commun.}}
@String{ wc     = "IEEE Wireless Commun."}
@String{ josaa  = {J.~Opt.~Soc.~Amer.~A}}
@String{ wn     = "Wireless Networks"}
@String{ ijgt   = "Intern. Journal of Game Theory"}
@String{ descon     = "Proc.~IEEE Conf.~on Design and Control"}
@String{ usc    = "University of Southern California"}
@String{ hermes     = "Hermes Penton Science"}
@String{ asilomar   = "Proc.~Asilomar Conf.~Signals, Systems, Comp."}
@String{ tnn    = {IEEE Trans.~Neural Networks}}
@String{ ett    = {European Trans.~Telecommun.}}
@String{ transcad   = "IEEE Trans.~CAD/ICAS"}
@String{ jlt    = {IEEE J.~Lightwave Tech.}}
@String{ plenum     = "Plenum Press"}
@String{ cp     = "Clarendon Press"}
@String{ tcomt  = {IEEE Trans.~Commun.~Technol.}}
@String{ melecon    = "Proc.~Mediterranean Electrotech. Conf."}
@String{ tcoms  = {IEEE Trans.~Commun.~Systems}}
@String{ mobicom    = "Proc.~ACM~Intern.~Conf. on Mobile Comput. and Networking (MOBICOM)"}
@String{ milcom     = "Proc.~IEEE Military Comm.~Conf. (MILCOM)"}
@String{ ton    = {IEEE/ACM Trans.~on Networking}}
@String{ tom    = {IEEE Trans.~Magnetics}}
@String{ toc    = {IEEE Trans. on~Commun.}}
@String{ tcom   = {IEEE Trans. on~Commun.}}
@String{ IEEE_J_COM   = {IEEE Trans. on~Commun.}}
@String{ siam   = {SIAM~J.}}
@String{ pi     = {Proc.~IEEE}}
@String{ athena     = "Athena Scientific"}
@String{ pimrc  = "Proc.~IEEE International Symposium on Personal, Indoor, and Mobile Radio Commun."}
@String{ spmag  = {IEEE Signal Processing Mag.}}
@String{ ol     = {Opt.~Lett.}}
@String{ ph     = "Prentice-Hall"}
@String{ springer   = "Springer-Verlag"}
@String{ isit   = "Proc.~Int. Symp. on Information Theory"}
@String{ towc   = "IEEE Trans.~on~Wireless~Comm."}
@String{ aap    = "Annals of Applied Prob."}
@String{ tap    = {IEEE Trans.~Antennas and Prop.}}
@String{ ai     = {Artif.~Intell.}}
@String{ ip     = "(In preparation)"}
@String{ ao     = "Applied Optics"}
@String{ ap     = "Academic Press"}
@String{ aw     = "Addison-Wesley"}
@String{ tac    = {IEEE Trans.~Automatic Control}}
@String{ nh     = "North-Holland"}
@String{ transelcomp    = "IEEE Trans.~Electronic Computers"}
@String{ istc   = "Proc. Intern. Symp. on Turbo Codes \& Relat. Topics"}
@String{ nl     = {Not Listed}}
@String{ nn     = {Neural Networks}}
@String{ tit    = {IEEE Trans.~Inform.~Theory}}
@String{ IEEE_J_IT    = {IEEE Trans.~Inform.~Theory}}
@String{ ieeeit    = {IEEE Trans.~Inform.~Theory}}
@String{ nc     = {Neural Computation}}
@String{ infocom    = "Proc.~IEEE Conf. on Computer Commun. (INFOCOM)"}
@String{ csp    = "Computer Science Press"}
@String{ fr     = "W. H. Freeman"}
@String{ wiley  = "John Wiley \& Sons"}
@String{ ios    = "IOS Press"}
@String{ kap    = "Kluwer Academic Publishers"}
@String{ ofc    = "Proc.~OFC"}
@String{ jwpc   = {J. Wireless Personal Commun.}}
@String{ globecom   = "Proc.~IEEE Global Telecommun. Conf."}
@String{ allerton   = "Proc.~Allerton~Conf.~Communications~Control~and~Computing"}
@String{ su     = "(Submitted)"}
@String{ aeu ={AEU Int. J.~Electron.~Commun.}}
@String{ ijscn   = "International~Journal~of~Satellite~Communications~and~Networking"}
@String{ wcnc   = "Proc.~IEEE~Wireless~Communications~and~Networking~Conf."}
@String{ istc   = "Proc.~Intl.~Symp.~Turbo~Codes~and~Rel.~Topics."}
@String{ jsstsp   = "Journal.~Sel.~Topics~in~Sig.~Proc."}
@String{ itw = "Proc.~IEEE~Inf.~Theory~Workshop"}

